Is your function low-dimensional?

We study the problem of testing if a function depends on a small number of linear directions of its input data. We call a function $f$ a linear $k$-junta if it is completely determined by some $k$-dimensional subspace of the input space. In this paper, we study the problem of testing whether a given $n$ variable function $f : \mathbb{R}^n \to \{0,1\}$, is a linear $k$-junta or $\epsilon$-far from all linear $k$-juntas, where the closeness is measured with respect to the Gaussian measure on $\mathbb{R}^n$. Linear $k$-juntas are a common generalization of two fundamental classes from Boolean function analysis (both of which have been studied in property testing) $\textbf{1.}$ $k$- juntas which are functions on the Boolean cube which depend on at most k of the variables and $\textbf{2.}$ intersection of $k$ halfspaces, a fundamental geometric concept class. We show that the class of linear $k$-juntas is not testable, but adding a surface area constraint makes it testable: we give a $\mathsf{poly}(k \cdot s/\epsilon)$-query non-adaptive tester for linear $k$-juntas with surface area at most $s$. We show that the polynomial dependence on $s$ is necessary. Moreover, we show that if the function is a linear $k$-junta with surface area at most $s$, we give a $(s \cdot k)^{O(k)}$-query non-adaptive algorithm to learn the function up to a rotation of the basis. In particular, this implies that we can test the class of intersections of $k$ halfspaces in $\mathbb{R}^n$ with query complexity independent of $n$.

==> testing-struct.tex <==
%\newcommand{\normal}{\mathcal{N}}
\red{
\section{Testing linear invariant subclasses of linear $k$-juntas} \label{sec:test-invariant}
In this section, we prove the following theorem. 
\begin{theorem}~\label{thm:test-invariant-struct}
 Let $\mathcal{C}$ be a collection of functions mapping $\mathbb{R}^k$ to $\{-1,1\}$. Further, for every $f \in \mathsf{Ind}(\mathcal{C})$, $\mathsf{surf}(f) \le s$. Then, there is an algorithm \textsf{Test-structure-$\mathcal{C}$} which has the following guarantee: Given oracle access to $f: \mathbb{R}^n \rightarrow \{-1,1\}$ and an error parameter $\epsilon>0$, the algorithm makes $(s \cdot k/\epsilon)^{O(k)}$ queries and distinguishes between the cases (i) $f \in \mathsf{Ind}(\mathcal{C})$ and (ii) $f$ is $\epsilon$-far from every function $f' \in \mathsf{Ind}(\mathcal{C})$. 
 \end{theorem} 
The algorithm \textsf{Test-structure-$\mathcal{C}$} is described in Figure~\ref{fig:tsi}. We now proceed with the proof of Theorem~\ref{thm:test-invariant-struct}. We begin with the following fact. 
\begin{figure}[tb]
\hrule
\vline
\begin{minipage}[t]{0.98\linewidth}
\vspace{10 pt}
\begin{center}
\begin{minipage}[h]{0.95\linewidth}
{\small
\underline{\textsf{Inputs}}
\vspace{5 pt}

\begin{tabular}{ccl}
$s$ &:=& surface area parameter \\
$\epsilon$ &:=& error parameter \\
%$S_{\mathsf{net}}$ &:=& the net of functions.\\
$k$ &:=& rank parameter\\
\end{tabular}


\underline{\textsf{Parameters}}
\vspace{5 pt}

\begin{tabular}{ccl}
$T_{inv}(s,k,\epsilon)$ &:=& query complexity of \textsf{Find-invariant-structure} with parameters $s$, $k$ and $\epsilon$.  \\
$\delta$ &:=& $(\epsilon / s \cdot k)^{O(k)}$ such that  $\delta \cdot T_{inv}(2s,k,\epsilon/4) \le \epsilon$. \\
%$S_{\mathsf{net}}$ &:=& the net of functions.\\
$k$ &:=& rank parameter\\
%$R$ &:=& Number of points where we evaluate each test function is evaluated\\
\end{tabular}



\vspace{5 pt}
\underline{\textsf{Testing algorithm}}
\begin{enumerate}
\item Run algorithm \textsf{Test-rank} with surface area parameter $s$, rank parameter $k$ and error parameter $\delta$. If \textsf{Test-rank} outputs no, output no. 
\item Otherwise, run routine \textsf{Find-invariant-structure} with surface area parameter $s$, rank parameter $k$ and error parameter $\epsilon/4$. 
\item Let $g: \mathbb{R}^\ell \rightarrow \{-1,1\}$ be the output of Step~2. Extend it to $\mathbb{R}^k$ where $g$ acts trivially in the last $n-k$ coordinates. Output yes if $g$ is $\epsilon$-close to some function in $\mathsf{Ind}(\mathcal{C})_k$. Otherwise, output no. 
\end{enumerate}

\vspace{5 pt}
}
\end{minipage}
\end{center}

\end{minipage}
\hfill \vline
\hrule
\caption{Description of the   algorithm \textsf{Test-Structure-$\mathcal{C}$}}
\label{fig:tsi}
\end{figure} 
\begin{fact}~\label{fact:unitary}
Let $f: \mathbb{R}^n \rightarrow \{-1,1\}$ be in $\mathsf{Ind}(\mathcal{C})$ defined as $f = g(\langle w_1, x \rangle, \ldots, \langle w_k, x\rangle)$ for $ g \in \mathcal{C}$ and orthonormal vectors $w_1, \ldots, w_k \in  \mathbb{R}^n$. If $v_1, \ldots, v_k$ is some other orthonormal basis of $\mathsf{span}(w_1, \ldots, w_k)$, then $f = \tilde{h}(\langle v_1, x \rangle, \ldots, \langle v_k ,x\rangle)$, for $\tilde{h} \in \mathsf{Ind}(\mathcal{C})_k$. 
\end{fact}
\begin{proof}
Observe that one go from the basis $(w_1, \ldots, w_k)$ to the basis $(v_1, \ldots, v_k)$ by means of a unitary transformation $U \in \mathbb{R}^{k \times k}$. Thus, $\tilde{h} =g \circ U$. However, observe that the function $\tilde{h}(x) = g \circ U (x)$ lies in $\mathsf{Ind}(\mathcal{C})_k$ which finishes the proof. 
\end{proof}



\begin{claim}~\label{clm:test-invariant-complete}
Assume that $f : \mathbb{R}^n \rightarrow \{-1,1\}$ is in $\mathsf{ind} (\mathcal{C})_n$. Further, $\mathsf{surf}(f) \leq s$. Then, $f$ passes \textsf{Test-Structure-$\mathcal{C}$} with probability $1-\epsilon$. 
\end{claim}
\begin{proof}
If $f \in \mathsf{ind} (\mathcal{C})_n$ with $\mathsf{surf}(f) \le s$, then \textsf{Test-rank} outputs yes with probability $1-\delta$. Let $w_1, \ldots, w_k$ be the implicit basis such that the output of Step~2 of \textsf{Test-Structure-$\mathcal{C}$} such that 
\[
\mathbf{E}[|g(\langle w_1, x \rangle, \ldots, \langle w_k, x \rangle) - f(x)|]  \le \frac{\epsilon}{4}. 
\]
As $f \in \mathsf{Ind}(\mathcal{C})$, there is an orthonormal set of vectors $(v_1, \ldots, v_k)$ and $h \in \mathcal{C}$ such that (i) $f = h(\langle v_1, x \rangle, \ldots, \langle v_k ,x \rangle)$ and (ii) $\mathsf{span}(w_1, \ldots, w_k) = \mathsf{span}(v_1, \ldots, v_k)$. By Fact~\ref{fact:unitary}, we get that there is a function $\tilde{h} \in \mathsf{Ind}(\mathcal{C})_k$ such that 
$f = \tilde{h}(\langle w_1, x\rangle, \ldots, \langle w_k, x\rangle)$. This implies that 
\[
\mathbf{E}[|g(\langle w_1, x\rangle, \ldots, \langle w_k, x\rangle)- \tilde{h}(\langle w_1, x\rangle, \ldots, \langle w_k, x\rangle)|] \le \frac{\epsilon}{4}. 
\]
Since $w_1, \ldots, w_k$ are orthonormal vectors, we get that $\mathbf{E}_{x \sim \gamma_k}[|g(x) - \tilde{h}(x)|] \le \frac{\epsilon}{4}$. This finishes the proof of the claim. 
\end{proof}

\begin{claim}~\label{clm:test-invariant-sound}
Assume that $f : \mathbb{R}^n \rightarrow \{-1,1\}$ is $\epsilon$-far from any function $f' \in \mathsf{Ind}(\mathcal{C})$. Then, the test \textsf{Test-Structure-$\mathcal{C}$} rejects with probability at least $0.9$. 
\end{claim}
\begin{proof}
First of all, if $f$ passes \textsf{Test-rank}  with probability $0.1$, then $f$ is $O(\delta)$-close to a linear $k$-junta $\tilde{f}$ with $\mathsf{surf}(\tilde{f}) \le (1+\delta) \cdot s$. Now, by Remark~\ref{rem:gaussian}, since the marginal of the queries made by the routine \textsf{Test-invariant-structure} is distributed as $\gamma_n$, hence with probability $1-O(\delta)$, we can assume that the queries are made to $\tilde{f}$. Note that the surface area of $\tilde{f}$ is at most $2s$. 
Since $\delta \cdot T_{inv}(2s,k,\epsilon/4) \le \epsilon$, hence with probability $1-\epsilon$, we can assume that the queries made by \textsf{Test-invariant-structure} are made to $\tilde{f}$. Then, with probability $1-2\epsilon$, Step~2 outputs a function $g$ such that there is an orthonormal set of vectors $w_1, \ldots, w_k$ and $h: \mathbb{R}^k \rightarrow \{-1,1\}$ with the following conditions: (i) $\mathbf{E}_{x \sim \gamma_k}[|g(\langle w_1, x\rangle, \ldots, \langle  w_k , x\rangle) - h(\langle w_1, x\rangle, \ldots, \langle  w_k , x\rangle)|] \le \frac{\epsilon}{4}$ and (ii) 
$\tilde{f} (x) = h(\langle w_1, x\rangle, \ldots, \langle  w_k , x\rangle)$. Let $g_0 \in \mathsf{Ind}(\mathcal{C})_k$ such that $g$ and $g_0$ are $\epsilon/4$-close. Because $w_1, \ldots, w_k$ are orthonormal, this also implies that 
$
\mathbf{E}_{x \sim \gamma_n}[|g(\langle w_1, x\rangle, \ldots, \langle  w_k , x\rangle) - g_0(\langle w_1, x\rangle, \ldots, \langle  w_k , x\rangle)|] \le \frac{\epsilon}{4}.
$ By applying triangle inequality, we get that 
\[
\mathbf{E}_{x\sim \gamma_n} [ |f(x) - g_0 (\langle w_1, x\rangle, \ldots, \langle w_k, x \rangle)|] \le \frac{\epsilon}{2} + O(\delta) \le\epsilon. 
\]
However, $g_0(\langle w_1, x\rangle, \ldots, \langle w_k, x \rangle) \in \mathsf{Ind}(\mathcal{C})_n$ contradicting the claim that $f$ is $\epsilon$-far from any function in $\mathsf{Ind}(\mathcal{C})$. 
\end{proof}
}
